Efficient and Accurate Learning of Mixtures of Plackett-Luce Models

Mixture models of Plackett-Luce (PL) -- one of the most fundamental ranking models -- are an active research area of both theoretical and practical significance. Most previously proposed parameter estimation algorithms instantiate the EM algorithm, often with random initialization. However, such an initialization scheme may not yield a good initial estimate and the algorithms require multiple restarts, incurring a large time complexity. As for the EM procedure, while the E-step can be performed efficiently, maximizing the log-likelihood in the M-step is difficult due to the combinatorial nature of the PL likelihood function (Gormley and Murphy 2008). Therefore, previous authors favor algorithms that maximize surrogate likelihood functions (Zhao et al. 2018, 2020). However, the final estimate may deviate from the true maximum likelihood estimate as a consequence. In this paper, we address these known limitations. We propose an initialization algorithm that can provide a provably accurate initial estimate and an EM algorithm that maximizes the true log-likelihood function efficiently. Experiments on both synthetic and real datasets show that our algorithm is competitive in terms of accuracy and speed to baseline algorithms, especially on datasets with a large number of items.

==> extra.tex <==



==> proofs/gap_proofs_old.tex <==
The following theorem shows that in the special case when $L = n$, the mixture model in Theorem \ref{thm:top-L-mixture-error-init} has a large inter-center gap (with high probability).

\begin{theorem}\label{thm:normal-random-mixture-model} Fix a constant number of mixture components $K$. Suppose that for mixture component $k\in [K]$, ${\theta^*}^k \sim \N(0, I_n)$.
There exists a constant $c >0$ such that
$$ \Delta_{\min} \geq \frac{c}{\sqrt{\log n}} \cdot \sqrt{n^2 - n\log n}  $$
with probability at least $1- \frac{K^2}{\poly(n)}$.
\end{theorem}

\begin{proof} We restrict our analysis to just two mixture components $\theta$ and $\theta'$ for now. To obtain the high probability guarantee for $K$ mixture components, a simple union bound argument suffices.

The mapping function under the case Plackett-Luce is exactly the link function for the BTL model. Specifically, for items $i, j$ with partworths ${\theta^*_i}, {\theta^*_j}$ respectively,
$$ P_{ij} = \frac{1}{1 + \exp{-({\theta^*_i} - {\theta_j^*})}} \,.$$
For now, consider just two mixture components with parameters ${\theta^*}$ and ${\theta^*}'$. The gap of their corresponding pairwise centers is
\begin{align*}
\Delta^2 &= \sum_{i < j} (P_{ij} - P'_{ij})^2\\
&\geq \sum_{i < j} l(\kappa)^2 \cdot \big(({\theta^*_i} - {\theta^*}) - ({\theta_i^*}' - {\theta_j^*}')\big)^2\,,
\end{align*}
where $l(\kappa)$ satisfies
$$\bigg\lvert\frac{1}{1 + \exp{-x}} - \frac{1}{1 + \exp{-y}} \bigg\rvert  \geq l(\kappa) \cdot \lvert x - y\rvert \,\forall \, x, y \in [-2\kappa, +2\kappa] \,.  $$
Clearly, $l(\kappa)$ is dependent on the dynamic range $\kappa$. Since the logit function is continuous everywhere, we can lower bound $l(\kappa)$ by lower bounding the gradient of the logit function within the dynamic range, which is
$$ \frac{\exp{-x}}{(1+\exp{-x})^2} $$
It is well known that for $\epsilon_1, \ldots, \epsilon_n \sim N(0, 1) $, $\max_i  \,\lvert \epsilon_i \rvert \leq 2C\sqrt{\log n}$ with probability $1 - O(\frac{1}{n^C})$. We have, for some constant $c' > 0$,
$$ l(\kappa) \geq \frac{\exp{-2C\sqrt{\log n}}}{(1+\exp{-2C\sqrt{\log n}})^2} \geq c'\,\exp{-2C\sqrt{\log n}}  $$
for $\kappa < 10\sqrt{\log n}$.
We will now tackle the remaining term in the expression for $\Delta^2$. We have
\begin{align*}
&\sum_{i < j} \big(({\theta_i^*} - {\theta_j^*}) - ({\theta_i^*}' - {\theta_j^*}')\big)^2\\
&= \frac{1}{2} \sum_{i \neq j}  \big(({\theta_i^*} - {\theta_j^*}) - ({\theta_i^*}' - {\theta_j^*}')\big)^2\\
&= \frac{1}{2} \sum_{i\neq j} \big( ({\theta_i^*} - {\theta_i^*}') - ({\theta_j^*} - {\theta_j^*}') \big)^2\\
&= \frac{1}{2} \sum_{i\neq j} ({\theta_i^*} - {\theta_i^*}')^2 + ({\theta_j^*} - {\theta_j^*}')^2 - 2({\theta_i^*} - {\theta_i^*}')({\theta_j^*} - {\theta_j^*}')\\
&= (n-1) \cdot \lVert {\theta^*} - {\theta^*}' \rVert_2^2 - ({\theta^*} - {\theta^*}')^\top (\mb 1_n \mb 1_n^\top - I_n) ({\theta^*} - {\theta^*}') \quad (*)\,. 
\end{align*}

~\\
We first bound the second order chaos term $({\theta^*} - {\theta^*}')^\top (\mb 1_n \mb 1_n^\top - I_n) ({\theta^*} - {\theta^*}')$. To this end, applying Theorem \ref{thm:hanson-wright} with $A = (\mb 1_n \mb 1_n^\top - I_n)$ suffices. Note that $A$ is indeed a diagonal free matrix with $\lVert A \rVert_{op} = n-1$ and $\lVert A \rVert_F = \sqrt{n^2-n}$. By Theorem \ref{thm:hanson-wright}, there exists a constant $c''$ such that
$$ \Pr\bigg(  \big\lvert ({\theta^*} - {\theta^*}')^\top (\mb 1_n \mb 1_n^\top - I_n) ({\theta^*} - {\theta^*}')  \big\lvert \geq t  \bigg) \leq \exp{-c''\min \bigg\{ \frac{t^2}{n^2}, \frac{t}{n} \bigg\}} \,. $$
For $t = 5n\log n$, $\frac{t}{n} \leq \frac{t^2}{n^2}$. We therefore have
$$ ({\theta^*} - {\theta^*}')^\top (\mb 1_n \mb 1_n^\top - I_n) ({\theta^*} - {\theta^*}') \leq \frac{5}{c''}\, n\log n\,. $$
with probability $1 - O(n^{-5})$. 

~\\
As for the $\lVert \theta^* - {\theta^*}'\rVert_2$ term, note that ${\theta^*} - {\theta^*}' \sim N(0, 2I_n)$. Applying Lemma \ref{lem:concentrate-norm} gives
 $$ \lVert {\theta^*} - {\theta^*}' \rVert^2_2 \geq \frac{5n}{c''} $$
with probability $1 - \exp{O(-n)}$.

~\\
Going back to the display $(*)$, we have
\begin{align*}
\Delta &\geq \frac{c'}{\log n} \cdot \sqrt{\frac{5n(n-1)}{c''} - \frac{5}{c''} n\log n}
\end{align*}
with probability at least $1 - O(n^{-5}) - O(\exp{-n})$. Applying union bound over all pairs of mixture components in $[K]$ gives us the conclusion in the theorem statement.
\end{proof}

The following theorem generalizes the above theorem to general $L$.
\begin{theorem}\label{thm:normal-top-L-random-mixture-model} Fix a constant number of mixture components $K$. Suppose that for mixture component $k\in [K]$, $\theta_{1:L}^{*k} \sim \N(0, I_L)$ and $\theta_{L+1:n}^{*k}=0$.
There exists a constant $c >0$ such that
$$ \Delta_{\min} \geq \frac{c}{\sqrt{\log n}} \cdot \sqrt{nL - L\log n}  $$
with probability at least $1- \frac{K^2}{\poly(n)} - O(K^2\exp{-L})$.
\end{theorem}

\begin{proof} Following the same argument as in the proof of Theorem \ref{thm:normal-random-mixture-model}, there exists a constant $c' > 0$ such that we decompose the gap between two cluster centers as
\begin{align*}
\Delta^2 &= \sum_{i < j} (P_{ij} - P'_{ij})^2\\
&\geq \sum_{i < j} l(\kappa)^2 \cdot \big(({\theta_i^*} - {\theta_j^*}) - ({\theta_i^*}' - {\theta_j^*}')\big)^2\,,\\
&= \bigg(\frac{c'}{\sqrt{\log n}}\bigg)^2 \cdot \bigg( (n-1) \cdot \lVert {\theta^*} - {\theta^*}' \rVert_2^2 - ({\theta^*} - {\theta^*}')^\top (\mb 1_n \mb 1_n^\top - I_n) ({\theta^*} - {\theta^*}') \bigg)\,. 
\end{align*}
Note that by design,
$$ {\theta^*} - {\theta^*}' = [({\theta^*} -{\theta^*}')_{1:L}, 0, \ldots, 0] \,.$$
Applying Lemma \ref{lem:concentrate-norm}, we have
$$ \lVert {\theta^*} -{\theta^*}' \rVert_2  = \lVert ({\theta^*} -{\theta^*}')_{1:L} \rVert_2 \gtrsim  \sqrt{L} $$
with probability at least $1 - O(\exp{-L})$. As for the second order chaos term, recall that because $\theta_{L+1:n} = \theta'_{L+1:n} = 0$, we have
\begin{align*}
&({\theta^*} - {\theta^*}')^\top (\mb 1_n \mb 1_n^\top - I_n) ({\theta^*} - {\theta^*}') \\
&= ({\theta^*} - {\theta^*}')_{1:L}^\top (\mb 1_L \mb 1_L^\top - I_L) ({\theta^*} - {\theta^*}')_{1:L} \,.
% &\lesssim L \sqrt{\log n}
\end{align*}
By Hanson-Wright's inequality (Theorem \ref{thm:hanson-wright}), there exists a constant $c''$ such that
$$ \Pr\bigg( \big\lvert ({\theta^*} - {\theta^*}')_{1:L}^\top (\mb 1_L \mb 1_L^\top - I_L) ({\theta^*} - {\theta^*}')_{1:L} \big\rvert \geq t \bigg) \leq 2 \,\exp{-c'' \cdot \min\{ \frac{t^2}{L^2}, \frac{t}{L} \}}\,.$$
For $t \gtrsim L\log n$, $\frac{t}{L} \lesssim \frac{t^2}{L^2}$.
Therefore,
$$ ({\theta^*} - {\theta^*}')_{1:L}^\top (\mb 1_L \mb 1_L^\top - I_L) ({\theta^*} - {\theta^*}')_{1:L}  \lesssim L\log n $$
with high probability (i.e., $1- O(\frac{1}{\poly(n)})$). The rest of the proof proceeds similarly to that of Theorem \ref{thm:normal-random-mixture-model}.
\end{proof}


==> proofs/spectral_init_proofs_old.tex <==
\textbf{Choice of $T$.} Theorem \ref{lem:operator-norm-bound} gives $\lVert E \rVert_{op} \lesssim \sqrt{n}({\sqrt m + \sqrt n})$. The technical condition in \citet{zhang2022leave} sugggests that $T$ is at least a constant factor larger than $\lVert E \rVert$. It therefore suffices to pick $T = \sqrt{n}\sqrt{m+n} \sqrt[4]{\log n}$. Additionally, the second bound in the theorem statement holds if
$$ \frac{\sqrt[4]{\log n} \, K^2 \lVert E\rVert_{op} }{\xi\sqrt m \Delta} = o(1)\,, $$ 
which can be satisfied under the generative model described in Theorem \ref{thm:top-L-mixture-error-init}. Define $\kappa$ to be the dynamic range, i.e., $\kappa := \max_{i\in[n], k\in[K]} \, \lvert \theta_i^{*k}\rvert$. In our generative model, $\kappa$ varies with $n$.
The rest of this section is devoted to showing that the inter-center gap $\Delta$ is sufficiently large under said generative model and Algorithm \ref{alg:spectral-clustering} enjoys exponentially decaying error rate as in Theorem \ref{thm:spectral-clustering}.

Let us introduce some notations. Let $C^{*k} = \{ l \in [m] \,\lvert \, z^*_l = k \}$ for $k\in [K]$ denote the true cluster assignment. To avoid cluttering the notation, let us suppress the relabeling operator here and consider $C^k = \{l \in [m] \,\lvert \, z_l = k \}$ to be the cluster assignment produced by Algorithm \ref{alg:spectral-clustering} corresponding to mixture component $k$.

\begin{reptheorem}{thm:top-L-mixture-error-init} (Corrected version) Consider a mixture of $K$ Plackett-Luce models with uniform mixing probabilities. Suppose that $\theta^{*k}_{i} = 0 \,\forall i \in [L+1:n]$ and $\theta^{*k}_{1:L} \sim \N(0, I_L)$ for $k\in [K]$. Suppose that $m\geq c\max \{K^4, Kn\}$ for a sufficiently large constant $c$. Then with high probability, the output $\btheta$ of Algorithm \ref{alg:spectral-init} satisfies the following for some constant $b$.
~\\
If $L \geq \exp{C \sqrt{\log n}}$ for a sufficiently large constant $C$, then
\begin{align*} \lVert \btheta - N(\btheta^*) \rVert_F &= O\bigg( \frac{\exp{b\sqrt{\log n}}\, \sqrt{K^2n\log n}}{\sqrt m} + \frac{\exp{b\sqrt{\log n}}\sqrt{nK}}{\exp{L}}\bigg)\\
&= O\bigg( K \cdot \sqrt{\frac{n^2\log n}{m}} + \frac{\sqrt K n}{e^{L}} \bigg)\,.
\end{align*}
If $L \geq C' n^\alpha$ for some constant $\alpha > 0$ and a sufficiently large constant $C'$, then
\begin{align*}
\lVert \btheta - N(\btheta^*) \rVert_F &= O\bigg(\exp{b\sqrt{\log n}} \frac{ \sqrt{K^2\, n\log n}}{\sqrt m} \bigg)\\
&= O\bigg( K\sqrt{\frac{n^2\log n}{m}}\, \bigg) 
\end{align*}
\end{reptheorem}

\begin{reptheorem}{thm:top-L-mixture-error-init} Consider a mixture of $K$ Plackett-Luce models with uniform mixing probabilities. Suppose that $\theta^{*k}_{i} = 0 \,\forall i \in [L+1:n]$ and $\theta^{*k}_{1:L} \sim \N(0, I_L)$ for $k\in [K]$. Suppose that $m\geq c\max \{K^4, Kn\}$ for a sufficiently large constant $c$. Then with high probability, the output $\btheta$ (modulo a relabeling of the mixture components) of Algorithm \ref{alg:spectral-init} satisfies the following for some constant $b$.
~\\
If $L \geq C \log^2 n$ for a sufficiently large constant $C$, then
\begin{align*} \lVert \btheta - N(\btheta^*) \rVert_F &= O\bigg( \frac{\exp{b\sqrt{\log n}}\, \sqrt{K^2n\log n}}{\sqrt m} + \frac{\exp{b\sqrt{\log n}}\sqrt{nK}}{\exp{\sqrt L}}\bigg)\\
&= O\bigg( K \cdot \sqrt{\frac{n^2\log n}{m}} + \frac{\sqrt K n}{e^{\sqrt L}} \bigg)\,.
\end{align*}
If $L \geq C' n^\alpha$ for some constant $\alpha > 0$ and a sufficiently large constant $C'$, then
\begin{align*}
\lVert \btheta - N(\btheta^*) \rVert_F &= O\bigg(\exp{b\sqrt{\log n}} \frac{ \sqrt{K^2\, n\log n}}{\sqrt m} \bigg)\\
&= O\bigg( K\sqrt{\frac{n^2\log n}{m}}\, \bigg) 
\end{align*}
\end{reptheorem}

\begin{proof} As noted before, when the mixing probabilities are uniform, $\beta^* = \frac{1}{K}\mb 1$, $\xi \approx 1$ and the size of each true cluster is $\approx \frac{m}{K}$ whp. In fact, for a cluster $k$, Hoeffding's inequality gives
$$ \Pr\bigg(\bigg\lvert \lvert C^{*k}\rvert - \frac{m}{K} \bigg\rvert > t \bigg) \leq 2 \,\exp{-\frac{2t^2}{m}} \,. $$
Hence, $\frac{0.9m}{K} \leq \lvert C^{*k} \rvert \leq \frac{1.1m}{K} $ with probability at least $1 - O(\exp{-m/K^2})$. Applying union bound over all clusters, gives
$$ \lvert C^{*k} \rvert \in \bigg[\frac{0.9m}{K}, \frac{1.1m}{K}\bigg] $$
with probability at least $1 - O(K\exp{-m/K^2})$.

~\\
Since the output of Algorithm \ref{alg:spectral-clustering} are $K$ clusters which are then used to estimate the pairwise preference probabilities -- the input to Algorithm \ref{alg:least-squares-estimate} -- it suffices to show that each pairwise center $\hat P^k$ is close to the corresponding true centers $P^{*k}$. 

~\\
Let us focus on a single cluster $k$. Recall the least squares loss function in Algorithm \ref{alg:least-squares-estimate}. When evaluated at the true parameter value $\theta^{*k}$, it is written as
\begin{align*}
\hat L(\theta^*) &= \sum_{i \neq j} \frac{1}{2} (\phi^k_{ji}- (\theta^{*k}_i - \theta^{*k}_j))^2 \,.
\end{align*}
The gradient is given as
\begin{align*}
(\nabla\hat L(\theta^{*k}))_i &= \sum_{j \neq i} (\phi^k_{ji}- (\theta_i^* - \theta_j^{*k}))(-1) + (\phi^k_{ij} - (\theta_j^{*k} - \theta^{*k}_i))\\
&= \sum_{j\neq i} \phi^k_{ij}-\phi^k_{ji} + 2(\theta_i^{*k} - \theta^{*k}_j) \\
&= \sum_{j\neq i} \phi^k_{ij}-\phi^{*k}_{ij} + \phi_{ji}^{*k} -\phi^k_{ji} + \underbrace{2(\theta^{*k}_i - \theta^{*k}_j) + \phi^{*k}_{ij} - \phi_{ji}^{*k}}_{=\, 0}  \\
&= \sum_{j\neq i}\phi^k_{ij}-\phi^{*k}_{ij} + \phi_{ji}^{*k} -\phi^k_{ji}
% &\lesssim e^{2\kappa} \cdot \sum_{j\neq i} \lvert P_{ij} - P^*_{ij} \rvert + \lvert P_{ji} - P^*_{ji} \rvert\\
% &\lesssim e^{2\kappa} n\sqrt{\log n}/\sqrt m
\end{align*}

~\\
From the above derivation, the first thing to note is that the derivative is translation invariant. That is $\nabla \hat L (\theta^{*k}) = \nabla \hat L (N(\theta^{*k}))$. Now, for $i, j$ where $i \neq j$, the second derivative is
\begin{align*}
\frac{\partial^2 \hat L(\theta^{*k})}{\partial \theta_i \partial \theta_j} &= -2\,.
\end{align*}
On the other hand,
\begin{align*}
\frac{\partial^2 \hat L(\theta^{*k})}{\partial \theta_i^2 } &= \sum_{j\neq i} 2 = 2(n-1)\,.
\end{align*}
Thus the Hessian of the loss function evaluated at $\theta^*$ is given as
$$ \hat H(\theta^{*k}) = 2n I_n - 2 \mb 1 \mb 1^\top \,.$$
In fact, $\hat H(\theta) = 2n I_n - 2 \mb 1 \mb 1^\top \forall \theta$. It is not hard to see that $\hat H(\theta) \mb 1 = 0$ (this is a consequence of the translation invariance of the utilities inherent in the PL/BTL model). The second eigen-value, however, is
$$\lambda_2 (H(\theta)) = n \,.$$


~\\
We now introduce the following fundamental argument from convex analysis that will provide a bound on $\lVert \theta^k - N(\theta^{*k})\rVert_2$
Define $\delta = \theta^k - N(\theta^{*k})$. It follows from the definition that $\delta$ is orthogonal to the all-one-vector. By convexity of the loss function $\hat L$ and the fact that $\theta^k$ is the minmimizer of $\hat L$, we have
$$ \hat L(\theta^k) \geq \hat L(\theta^{*k}) + \langle \nabla L(\theta^{*k}), \delta \rangle\,. $$
Consequently,
$$ \hat L(\theta^{*k}) - \hat L(\theta^k) - \langle \nabla L(\theta^{*k}), \delta \rangle \leq \langle \nabla L(\theta^{*k}), -\delta\rangle \leq \lVert \nabla \hat L(\theta^{*k})\rVert_2 \, \lVert \delta \rVert_2 $$
% $$ \hat L(\theta^k) - \hat L(\theta^{*k}) - \langle\nabla \hat L(\theta^{*k}, \delta) \rangle \geq -\langle \nabla \hat L(\theta^{*k}, \delta) \geq - \lVert \nabla \hat L(\theta^*)\rVert_2 \lVert \delta \rVert_2 \,.$$
On the other hand, by Taylor expansion, there exists some $\theta$ which is a convex combination of $\theta^{*k}$ and $\theta^k$ such that
$$ \hat L(\theta^k) - \hat L(\theta^*) - \langle\nabla \hat L(\theta^{*k}, \delta) \rangle = \frac{1}{2} \delta^2 H(\theta) \delta \geq \frac{1}{2}\,\lambda_2(\hat H(\theta)) \lVert \delta \rVert_2^2 \,.$$
Combining the above two bounds gives
\begin{equation}\label{eqn:ell2-bound}
\lVert \delta\rVert_2 \leq \frac{2\lVert \nabla \hat L(\theta^*)\rVert_2}{\lambda_2(\hat H(\theta))} = \frac{\lVert \nabla \hat L(\theta^*)\rVert_2}{n}
\end{equation}
The rest of the proof is devoted to obtaining a bound on $\lVert \hat L(\theta^*)\rVert_2$.

~\\
Before analyzing the norm of the derivative, however, let us introduce a quantity $\bar l(\kappa)$ (not to be confused with $l(\kappa)$ introduced earlier) where for any $x, y \in [-2\kappa, 2\kappa]$
$$ \bigg\lvert \ln\bigg(p/(1-p)\bigg) - \ln\bigg(p'/(1-p') \bigg) \bigg\rvert \leq \bar l(\kappa) \cdot \lvert p - p'\rvert\,. $$ 
Essentially, $\bar l(\kappa)$ is the Lipschitz `constant' for the transformation function $\ln(p/(1-p))$ under the dynamic range $\kappa$. Since the logit function is continuous, we can bound its lipschitz constant by bounding the absolute value of the gradient of the logit function. It can be checked that the gradient is
$$  \frac{1}{p} + \frac{1}{1-p}\,. $$
When $\lvert \theta_i^{*k} \rvert \lesssim \sqrt{\log n}$, one can check that $1/P_{ij}^{*k} \lesssim \exp{\sqrt{\log n}}$.

~\\
Focusing on a single pair $(i, j)$, let $N^k_{ij}$ denote the number of times that item $j$ `beats' item $i$ among the permutations in cluster $\hat C^k$.
\begin{align*}
N^k_{ji} &= \sum_{l\in C^{*k}} \ind [\pi_l(i) < \pi_l(j)] - \sum_{l\in C^{*k}, l\notin \hat C^k} \ind [\pi_l(i) < \pi_l(j)] + \sum_{l \notin C^{*k}, l\in \hat C^k} \ind [\pi_l(i) < \pi_l(j)]\,.
% &\asymp m P_{ji}^* \pm O(\sqrt{m\log n}) \pm m \cdot O\bigg( \exp{-\frac{\Delta^2}{\sigma^2}} + \exp{-m} \bigg)
\end{align*}
We will analyze these terms separately. By Hoeffding's inequality, the first term can be bounded as
\begin{align*}
\Pr\bigg(\bigg\lvert \sum_{l\in C^{*k}} \ind [\pi_l(i) < \pi_l(j)] - \lvert C^{*k} \rvert \cdot P_{ij}^*\bigg\lvert > t \bigg) \leq 2\exp{-\frac{2t^2}{ \lvert C^{*k}\rvert }} \leq  2\exp{-\frac{2K\,t^2}{ 1.1m}}  \,.
\end{align*}
Therefore,
$$\big\lvert \sum_{l\in C^k} \ind [\pi_l(i) < \pi_l(j)] - \lvert C^k \rvert \cdot P_{ij}^*\big\lvert  \lesssim \sqrt{m/K \, \log n} $$
with high probability (i.e., at least $1 - O(\frac{1}{\poly(n)}))$.

~\\
Note that by definition,
\begin{align*}
\bigg\lvert \sum_{l\in C^k, l\notin \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \bigg\rvert + \bigg\lvert \sum_{l \notin C^k, l\in \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \bigg\rvert \leq m \cdot \ell(z, z^*)\,.
\end{align*}

~\\
Under the assumptions stated in the theorem, the output of Algorithm \ref{alg:spectral-clustering} achieves exponentially decaying mis-clustering error rate and
\begin{align*}
&\Pr\bigg(  \bigg\lvert \sum_{l\in C^k, l\notin \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \bigg\rvert + \bigg\lvert \sum_{l \notin C^k, l\in \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \bigg\rvert  > t \bigg)\\
&\leq \Pr\bigg( m\cdot \ell(z, z^*) > t \bigg) =  \Pr\bigg(\ell(z, z^*) > \frac{t}{m} \bigg) \\
&\leq\frac{m}{t} \cdot \exp{-(1- C'(\rho\psi^{-1}+\rho^{-1})) \frac{\Delta^2}{8\sigma^2} } + \frac{m}{t} \cdot \exp{-\frac{m}{2}} \quad(*) \,,
\end{align*}
where the last step comes from applying Markov's inequality and $\psi, \rho, C'$ are defined in Theorem \ref{thm:spectral-clustering}.


~\\
At this point, we consider the two regimes of $L$ separately as the first term in the display $(*)$ will differ substantially between the two regimes.

~\\
\textbf{For the regime $L \asymp \log^2 n$}, Theorem \ref{thm:normal-random-mixture-model} gives
$$ \Delta_{\min} \gtrsim \frac{1}{\sqrt{\log n}} \cdot \sqrt{nL - L\log n} \asymp \sqrt{\frac{L}{\log n} \cdot (n - \log n)} \asymp \sqrt{\log n(n-\log n)} \,. $$
One can verify that the ratio $\rho/\psi$ in Theorem \ref{thm:spectral-clustering} satisfies
$$ \frac{\sqrt[4]{\log n} \, K^2 \lVert E\rVert_{op} }{\xi\sqrt m \Delta} \asymp \frac{\sqrt[4]{\log n} \, K^2 \sqrt n \sqrt{m+n} }{\sqrt m \sqrt{\log n} \,\sqrt{n}} = o(1)\,.$$ 
As a result, the first term in the display $(*)$ can be bounded as
\begin{align*}
\exp{-(1- C'(\rho\psi^{-1}+\rho^{-1})) \frac{\Delta^2}{8\sigma^2} } \leq \exp{-(1-o(1)) \cdot \frac{\Delta^2}{8n}}
% &\leq \frac{m}{t} \cdot \exp{-(1-o(1)) \cdot c_L \cdot \frac{L}{\log n} \cdot \underbrace{(1 - \log n/n)}_{= \, (1-o(1))} }\\
% &= \frac{m}{t} \cdot \exp{-(1-o(1)) \cdot c_L  \cdot \frac{L}{\log n} }\\
% &= m \cdot \exp{-(1-o(1)) \cdot c_L  \cdot \frac{L}{\log n} + \log\big(\frac{1}{t}\big)}\,.
\end{align*}
Substitute $t = \frac{m}{Kn}$ into the display $(*)$. There exists a constant $c_L > 0$ such that
\begin{align*}
&\Pr\bigg(  \bigg\lvert \sum_{l\in C^k, l\notin \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \bigg\rvert + \bigg\lvert \sum_{l \notin C^k, l\in \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \bigg\rvert  > {\frac{m}{K e^{\sqrt L} }} \bigg)\\
&\leq Ke^{\sqrt L} \cdot \exp{-(1-o(1)) \cdot c_L \cdot \frac{L}{\log n}} + Kn \cdot \exp{-\frac{m}{2}} \\
&= K  \cdot \exp{-(1-o(1)) \cdot c_L \cdot \frac{L}{\log n} +\sqrt{L} } + Kn \cdot \exp{-\frac{m}{2}} \\
&[\text{Suppose that $L \geq C\log^2 n$ for a sufficiently large constant $C$. }]\\
&\leq \frac{K}{\poly(n)} + \frac{Kn}{e^{-m/2}} \quad (**)
\end{align*}

~\\
By the assumption that $m\geq Kn$, the $ \frac{Kn}{e^{-m/2}} \lesssim \frac{1}{\poly(n)}$. 
We thus have, with high probability (at least $1- O(\frac{1}{\poly(n)})$),
$$ \bigg\lvert N_{ij} - \frac{m}{K} \cdot P_{ij}^{*k} \bigg\rvert \lesssim \sqrt{m/K \, \log n} + m \ell(z, z^{*}) \asymp \sqrt{m/K \, \log n}  + \frac{m}{Ke^{\sqrt L}} \,.$$
Since $ C^{*k} \asymp \frac{m}{K}\, $ and $ \lvert \hat C^k - C^{*k} \rvert \leq  \frac{m}{Kn}\,, $ we have $\hat C^k \asymp \frac{m}{K}$.

~\\
Consequently,
\begin{align*}
\lvert \hat P^k_{ij} - P^{*k}_{ij} \rvert =\bigg\lvert \frac{N^k_{ij}}{\lvert \hat C^k\rvert} - P_{ij}^* \bigg\rvert \asymp \frac{1}{m/K} \cdot \bigg\lvert N^k_{ij} - {m/K} \cdot {P^*_{ij}}  \bigg\rvert  \lesssim \frac{\sqrt K\,\sqrt{\log n}}{\sqrt m} + \frac{1}{e^{\sqrt L}} \,.
\end{align*}

~\\
So long as the probability bound in $(**)$ is small enough, which is satisfied when $C$ is sufficiently large, then we can apply union bound over all pairs $i\neq j$ and still have
$$ \lvert P^k_{ij} - P^{*k}_{ij} \rvert \lesssim  \frac{\sqrt K \, \sqrt{\log n}}{\sqrt m} + \frac{1}{e^{\sqrt L}} $$
hold for all pairs $i,j$ with high probability.

~\\
We can now bound the norm of the derivative of $\hat L$ at $\theta^{*k}$ as
\begin{align*}
\lVert \nabla\hat L(\theta^*)\rVert_2^2 &= \sum_i (\sum_{j\neq i} ( \phi^k_{ij}-\phi_{ij}^{*k} + \phi_{ji}^{*k} - \phi^k_{ji} ))^2\\
&\leq \sum_i\bigg(\sum_{j\neq i} \bar l(\kappa) \cdot \big(\lvert P^k_{ij}- P^{*k}_{ij}\rvert + \lvert P_{ji}^{*k} - P^k_{ji}\rvert\big) \bigg)^2\\
&\lesssim \sum_i \bigg(\sum_{j\neq i} \exp{O(\sqrt{\log n})}\cdot \bigg(\frac{\sqrt K\sqrt{\log n}}{\sqrt m} + \frac{1}{e^{\sqrt L}} \bigg) \bigg)^2\\
&\asymp n^3 \bigg(\frac{\exp{O(\sqrt{\log n})}\, \sqrt K \sqrt{\log n}}{\sqrt m} + \frac{\exp{O(\sqrt{\log n})}}{e^{\sqrt L}}\bigg)^2\,.
\end{align*}
Taking the square root of both sides gives
$$ \lVert \nabla \hat L(\theta^*)\rVert_2 \lesssim n\sqrt n \cdot  \bigg(\frac{\exp{O(\sqrt{\log n})}\, \sqrt K \sqrt{\log n}}{\sqrt m} + \frac{\exp{O(\sqrt{\log n})}}{e^{\sqrt L}}\bigg) \,. $$
Applying Inequality (\ref{eqn:ell2-bound}) gives
\begin{align*}
\lVert \theta^k - {\theta^*}^k \rVert_2 &\leq \frac{\lVert \nabla \hat L(\theta^*)\rVert_2  }{n}\\
&\lesssim \sqrt n\cdot  \bigg(\frac{\exp{O(\sqrt{\log n})}\, \sqrt K \sqrt{\log n}}{\sqrt m} + \frac{\exp{\sqrt{\log n}}}{e^{\sqrt L}}\bigg) \\
&\asymp \frac{\exp{O(\sqrt{\log n})}\, \sqrt K \sqrt{n\log n}}{\sqrt m} + \frac{\exp{O(\sqrt{\log n})}\sqrt n}{e^{\sqrt L}} \,.
\end{align*}

~\\
\textbf{For the regime $L \asymp n^\alpha$.} Pick $L = C n^{\alpha}$ for some constant $C$ to be determined later. Theorem \ref{thm:normal-random-mixture-model} gives
$$ \Delta_{\min} \gtrsim \frac{1}{\sqrt{\log n}} \cdot \sqrt{nL - L\log n} \asymp \sqrt{\frac{Cn^\alpha}{\log n} \cdot (n - \log n)} \,. $$
Again, one can check that $\rho/\psi = o(1)$ (which is more easily satisfiable than the regime $L \asymp \log^2 n$).
Therefore, the first term in $(*)$ can be bounded as
\begin{align*}
\cdot \exp{-(1- C'(\rho\psi^{-1}+\rho^{-1})) \frac{\Delta^2}{8\sigma^2} } \leq \frac{m}{t} \cdot \exp{-(1-o(1)) \frac{\Delta^2}{8n}}
% &\leq \frac{m}{t} \cdot \exp{-(1-o(1)) \cdot c \cdot \frac{Cn^\alpha}{\log n} \cdot (1 - \log n/n) }\\
% &= \frac{m}{t} \cdot \exp{-(1-o(1)) \cdot c \cdot \frac{Cn^\alpha}{\log n} }\\
% &= m \cdot \exp{-(1-o(1))\cdot c \cdot \frac{Cn^\alpha}{\log n} + \log\big(\frac{1}{t}\big)}\,.
\end{align*}
Substituting $t = \frac{1}{\sqrt{m/K}}$ into the display $(*)$, we have
\begin{align*}
&\Pr\bigg(  \lvert \sum_{l\in C^k, l\notin \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \rvert + \lvert \sum_{l \notin C^k, l\in \hat C^k} \ind [\pi_l(i) < \pi_l(j)] \rvert  > \frac{m}{\sqrt{mK}} \bigg)\\
&\leq \sqrt{mK} \cdot \exp{-(1-o(1)) \cdot c \cdot \frac{Cn^\alpha}{\log n}} + \sqrt{mK} \cdot \exp{-\frac{m}{2}} \\
&\leq \sqrt{K} \cdot \exp{-(1-o(1)) \cdot c \cdot \frac{Cn^\alpha}{\log n} + 1/2 \, \log m} + \sqrt{mK} \cdot \exp{-\frac{m}{2}} 
\end{align*}

~\\
Assuming that $m = o(e^n)$, then for a sufficiently large $C$, the first exponential term in the display above can be bounded as
$$\exp{-(1-o(1)) \cdot c \cdot \frac{Cn^\alpha}{\log n} + 1/2 \, \log m} \leq \frac{1}{\exp{n^{\alpha}}}\,.$$ 
The second term $\sqrt{mK} \cdot \exp{-m/2}$ decays exponentially fast with $m$ and is dominated by the first term.
We have with probability $1 - O(\exp{-n^{\alpha}})$
$$ \bigg\lvert N_{ij} - \frac{m}{K} \cdot P_{ij}^{*k} \bigg\rvert \lesssim \sqrt{m/K \, \log n} + m \ell(z, z^{*}) \asymp \sqrt{m/K \, \log n}  + \sqrt{m/K} \,.$$
Since $ C^{*k} \asymp \frac{m}{K}\, $ and $ \lvert \hat C^k - C^{*k} \rvert \leq  \sqrt{\frac{m}{K}} \,, $ we have $\hat C^k \asymp \frac{m}{K}$.

~\\
Following similar arguments as for the earlier case of $L \asymp \poly\log n$, we have with high probability, the following holds for all pairs $i, j$ with high probability.
\begin{align*}
\lvert \hat P^k_{ij} - P^{*k}_{ij} \rvert =\bigg\lvert \frac{N^k_{ij}}{\lvert \hat C^k\rvert} - P_{ij}^* \bigg\rvert \asymp \frac{1}{m/K} \cdot \bigg\lvert N^k_{ij} - m/K \cdot P^*_{ij}  \bigg\rvert  \lesssim \frac{\sqrt K\,\sqrt{\log n}}{\sqrt m} + \frac{\sqrt K}{\sqrt m} \,.
\end{align*}

~\\
We can now bound $\lVert \nabla \hat L(\theta^{*k})$ as follows
\begin{align*}
\lVert \nabla\hat L(\theta^{*k})\rVert_2^2 &= \sum_i (\sum_{j\neq i} ( \phi^k_{ij}-\phi_{ij}^{*k} + \phi_{ji}^{*k} - \phi^k_{ji} ))^2\\
&\leq \sum_i\bigg(\sum_{j\neq i} \bar l(\kappa) \cdot \big(\lvert P^k_{ij}-P_{ij}^{*k}\rvert + \lvert P_{ji}^{*k} - P^k_{ji}\rvert\big) \bigg)^2\\
&\lesssim \sum_i \bigg(\sum_{j\neq i} \exp{O(\sqrt{\log n})} \cdot \bigg(\frac{\sqrt K\sqrt{\log n}}{\sqrt m} + \frac{\sqrt K}{\sqrt m}\bigg) \bigg)^2\\
&\asymp n^3  \bigg(\exp{O(\sqrt{\log n})}\frac{\sqrt K \sqrt{\log n}}{\sqrt m} \bigg)^2\,.
\end{align*}
Taking the square root of both sides gives
$$ \lVert \nabla \hat L(\theta^*)\rVert_2 \lesssim n \sqrt n \cdot \exp{\sqrt{\log n}} \cdot \frac{\sqrt K\sqrt{\log n}}{\sqrt m} \,. $$
Finally, we apply Inequality (\ref{eqn:ell2-bound}) to obtain
\begin{align*}
\lVert \theta^k - {\theta^*}^k \rVert_2 &\leq \frac{\lVert \nabla \hat L(\theta^*)\rVert_2  }{n} \lesssim \sqrt n\cdot  \exp{O(\sqrt{\log n})} \cdot \frac{\sqrt K\sqrt{\log n}}{\sqrt m} \\
&\asymp \exp{O(\sqrt{\log n})} \frac{\sqrt K \sqrt{n\log n}}{\sqrt m} \,.
\end{align*}

~\\
\textbf{Putting things together.} The theorem statements are obtained by first noting that $\exp{O(\sqrt{\log n})}\lesssim \exp{\frac{1}{2} \log n} \lesssim \sqrt n$. In fact $\exp{O(\sqrt{\log n})}$ grows slower, asymptotically, than any $n^u$ for $u > 0$. But to obtain the theorem statement, bounding $\bar l$ as follows suffices.
$$ \bar l \lesssim \sqrt n \,.$$
Lastly,
$$ \lVert \btheta - \btheta^* \rVert_f \leq \sqrt K \cdot \max_{k} \, \lVert \theta^k - \theta^{*k}\rVert_2\,. $$
This finishes the proof.
\end{proof}
